Fully Convolutional Multi-scale Residual DenseNets for Cardiac Segmentation and Automated Cardiac Diagnosis using Ensemble of Classifiers

Deep fully convolutional neural network (FCN) based architectures have shown great potential in medical image segmentation. However, such architectures usually have millions of parameters and inadequate number of training samples leading to over-fitting and poor generalization. In this paper, we present a novel highly parameter and memory efficient FCN based architecture for medical image analysis. We propose a novel up-sampling path which incorporates long skip and short-cut connections to overcome the feature map explosion in FCN like architectures. In order to processes the input images at multiple scales and view points simultaneously, we propose to incorporate Inception module's parallel structures. We also propose a novel dual loss function whose weighting scheme allows to combine advantages of cross-entropy and dice loss. We have validated our proposed network architecture on two publicly available datasets, namely: (i) Automated Cardiac Disease Diagnosis Challenge (ACDC-2017), (ii) Left Ventricular Segmentation Challenge (LV-2011). Our approach in ACDC-2017 challenge stands second place for segmentation and first place in automated cardiac disease diagnosis tasks with an accuracy of 100%. In the LV-2011 challenge our approach attained 0.74 Jaccard index, which is so far the highest published result in fully automated algorithms. From the segmentation we extracted clinically relevant cardiac parameters and hand-crafted features which reflected the clinical diagnostic analysis to train an ensemble system for cardiac disease classification. Our approach combined both cardiac segmentation and disease diagnosis into a fully automated framework which is computational efficient and hence has the potential to be incorporated in computer-aided diagnosis (CAD) tools for clinical application.

==> redundant.tex <==
% \begin{table}
% \parbox{.103\textwidth}{
% \centering
% \caption*{\textbf{Layer}}
% \begin{tabular}{|c|ll}
% \cline{1-1}
% Batch Normalization      &  &  \\ \cline{1-1}
% Exponential Linear Unit         &  &  \\ \cline{1-1}
% $3 \times 3$ Convolution &  &  \\ \cline{1-1}
% Dropout $p = 0.2$        &  &  \\ \cline{1-1}
% \end{tabular}
% }
% \hfill
% \parbox{.103\textwidth}{
% \centering
% \caption*{\textbf{TD}}
% \begin{tabular}{|c|ll}
% \cline{1-1}
% Batch Normalization      &  &  \\ \cline{1-1}
% Exponential Linear Unit         &  &  \\ \cline{1-1}
% $1 \times 1$ Convolution &  &  \\ \cline{1-1}
% Dropout $p = 0.2$        &  &  \\ \cline{1-1}
% $2 \times 2$ Max Pooling        &  &  \\ \cline{1-1}
% \end{tabular}
% }
% \hfill
% \parbox{.103\textwidth}{
% \centering
% \caption*{\textbf{TU}}
% \begin{tabular}{|c|ll}
% \cline{1-1}
% $3 \times 3$ Transposed \\Convolution\\
% stride = 2     &  &  \\ \cline{1-1}
% \end{tabular}
% }
% \caption{Building blocks of DFCN. From left to right: layer used in the model, Transition Down (TD) and Transition
% Up (TU).}
% \label{tab:bloc}
% \end{table}
 

% \begin{table}[h]
% \centering
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{c}
% \hline
% \multicolumn{1}{|c|}{{\textbf{DFCN Architecture}}}                                                                                                         \\ \hline
% \multicolumn{1}{l}{}                                                                                                                                      \\ \hline
% \multicolumn{1}{|c|}{Input\_Size: ($128\times128$),  channels=1}                                                                                          \\ \hline
% \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Inception\_X:\\  $3\times3$ (16), $5\times$5 (8), $7\times7$ (8) convolutions, features = 32\end{tabular}} \\ \hline
% \multicolumn{1}{|c|}{DB (3 layers) + TD, features = 56}                                                                                 \\ \hline
% \multicolumn{1}{|c|}{DB (4 layers) + TD, features = 88}                                                                                 \\ \hline
% \multicolumn{1}{|c|}{DB (5 layers) + TD, features = 128}                                                                                \\ \hline
% \multicolumn{1}{|c|}{Short Skip + Bottleneck (8 layers), features = 64}                                                                                     \\ \hline
% \multicolumn{1}{|c|}{TU + Long Skip + DB (5 layers) + Short Skip, features = 40}                                                                                  \\ \hline
% \multicolumn{1}{|c|}{TU + Long Skip + DB (4 layers) + Short Skip, features = 32}                                                                                  \\ \hline
% \multicolumn{1}{|c|}{TU + Long Skip + DB (3 layers) + Short Skip, features = 24}                                                                                    \\ \hline
% \multicolumn{1}{|c|}{$1\times1$ convolution, channels = 4}                                                                                                  \\ \hline
% \multicolumn{1}{|c|}{Softmax Layer}                                                                                                                       \\ \hline
% \textbf{Number of Dense Convolutional layers : 50}                                                                                                              \\
% \textbf{Number of parameters : 331332}                                                                                                                   
% \end{tabular}%
% %  }
% \caption{Architecture details of model used in our experiments. The growth rate parameter \textbf{$k=8$}}
% \label{tab:arch}
% \end{table}



